Moment Preserving Constrained Resampling with Applications to Particle-in-Cell Methods

In simulations of partial differential equations using particle-in-cell (PIC) methods, it is often advantageous to resample the particle distribution function to increase simulation accuracy, reduce compute cost, and/or avoid numerical instabilities. We introduce an algorithm for particle resampling called Moment Preserving Contrained Resampling (MPCR). The general algorithm partitions the system space into smaller subsets and is designed to conserve any number of particle and grid quantities with a high degree of accuracy (i.e. machine accuracy). The resampling scheme can be integrated into any PIC code. The advantages of MPCR, including performance, accuracy, and stability, are presented by examining several numerical tests, including a use-case study in gyrokinetic fusion plasma simulations. The tests demonstrate that while the computational cost of MPCR is negligible compared to the nascent particle evolution in PIC methods, periodic particle resampling yields a significant improvement in the accuracy and stability of the results.

==> Makefile <==
all:	all_texs

clean: clean_texs clean_exec

clean_texs:
	rm -f *.aux
	rm -f *.log
	rm -f *.dvi
	rm -f *.toc
	rm -f *.blg
	rm -f *.idx
	rm -f *.pdf
	rm -f .DS_Store
	rm -f paper_0_main*.ps
	rm -f *.out
	rm -f *.nav
	rm -f *.synctex.gz
	rm -f *.snm

clean_exec:
	rm -f *~

#OBJS_convert = \
#	rawfigs/xyz.eps \
#	rawfigs/abc.eps

# $(OBJS_convert)

all_texs:
	pdflatex paper_0_main.tex
	pdflatex paper_0_main.tex
	bibtex   paper_0_main
	pdflatex paper_0_main.tex
	pdflatex paper_0_main.tex


.SUFFIXES: .eps .png .jpg

%.eps: %.png
	convert $< $(basename $<).eps

%.eps: %.jpg
	convert $< $(basename $<).eps


==> paper_2_gyro.tex <==
%% The main motivation of the general purpose resampling algorithm presented in this paper is to improve solution accuracy of PIC gyrokinetic codes in various applications of plasma simulation.
%% To provide
%% context for this algorithmic development, the PIC methods are described briefly in this section.

%% The kinetic theory of collisional plasmas can be used to describe the
%% behavior of gases and plasmas in terms of the motion of atomic
%% particles (ions and electrons). Particle motion is represented
%% by the evolution of the particle distribution functions
%% $f(\mathbf{x},\mathbf{v},t)$, depending on position $\mathbf{x}$, velocity $\mathbf{v}$, and time $t$.
%% Thus, in general case, the distribution functions measure the number density of
%% atomic particles in a six-dimensional phase space
%% $(\mathbf{x},\mathbf{v})$.  
%% %
%% The evolution of the $f$'s for various
%% atomic species is described by a multi-species 
%% Boltzmann equation coupled to classical electrodynamics
%% (i.e. Maxwell's equations).
%% As an example, we consider 
%% electrostatic perturbations,
%% by essentially replacing Maxwell's equations with Gauss's law.
%% %
%% For a given charged species this system can
%% be written as:
%% \begin{equation}\begin{aligned}\label{eq:boltzmann}
%% \frac{\partial f}{\partial t} + \mathbf{v} \frac{\partial f}{\partial \mathbf{x}} + \frac{q}{m} (\mathbf{E}+\mathbf{v}\times\mathbf{B}) \frac{\partial f}{\partial \mathbf{v}} = C(f) + S, \quad \nabla\cdot\mathbf{E}  & = -G,
%% \end{aligned}\end{equation} 
%% where $\mathbf{E}$ is the electric field, $\mathbf{B}$ the magnetic
%% field, $C$ a collisional operator describing sub-grid Coulomb interactions,
%% $S$ a source and sink term, $G$ a forcing (net charge) for the
%% electrostatics, and $q$ is the charge and $m$ is mass of species.
%% %
%% The electric and magnetic fields are determined by Maxwell equations 
%% \begin{eqnarray}\label{eq:maxwell}
%% \boldsymbol{\nabla} \times \mathbf{B}&-&\frac{1}{c^2}\frac{\partial\mathbf{E}}{\partial t}  = \mu_0 \mathbf{J} \\ 
%% \boldsymbol{\nabla} \times \mathbf{E}&+& \frac{\partial\mathbf{B}}{\partial t}  = 0\\
%% \boldsymbol{\nabla} \cdot \mathbf{E}  &=& \frac{\rho}{\epsilon_0} \\
%% \boldsymbol{\nabla} \cdot \mathbf{B}  &=& 0 ,
%% \end{eqnarray}
%% where $\rho$ is charge density, $\mathbf{J}$ is the current density, $\epsilon_0$ and $\mu_0$ are called the permittivity and permeability of vacuum, and $c = 1/\sqrt{\epsilon_0 \mu_0}$
%% is the speed of light.

% defining PIC
The Particle-in-Cell (PIC) method has been incredibly successful for solving large classes of differential equations in many application areas.  Though the numerical properties of PIC render it sensitive to discrete particle noise and instability, it excels in generating unusually robust and exceedingly parallelizable representations of complex systems.  In the PIC method, the distribution function $f$ is sampled and the evolution of $f$ is represented by the evolution of the samples in the system space (e.g. the phase space in statistical mechanics). The samples are called particles, marker particles, macro-particles, or sometimes superparticles and are essentially a Lagrangian representation of the evolution of $f$. The coupled field solvers, on the other hand, are generally solved over an Eulerian grid based on finite difference \cite{westermann1994}, finite volume \cite{Hermeline2008}, and/or finite element \cite{Assous1993} discretizations.  In standard PIC methods, the particles are deposited from the position of the computational particles to the grid nodes, then the field solver is run using the particle data as part of the forcing, and finally, the grid field is scattered back to the particle positions and used to propagate the solution of particles equations of motion. 

The objective of PIC methods is to represent $f$ using orders of magnitude fewer marker particles than physical atomic particles. For this reason, each marker particle carries a weight so that the sum of the weights over all the marker particles gives the number of physical
particles. The marker particles can also be non-uniformly weighted for importance sampling, which allows more samples (particles) to be used to represent important parts of the phase space. For example, more particles with smaller weights can be used in low-density regions to
provide a good representation of these regions. More particles can also be used in the high energy space when they become important. Considering one realization of a volume filled with particles in phase space, the PIC method approximates the distribution function as a combination of Dirac delta functions (called the Klimontovich density), 
%
\begin{eqnarray}\label{eq:f_dist}
f(\mathbf{x}, \mathbf{v}, t) &\approx&  \sum_{j=1}^{N^p} w_j \delta (\mathbf{x}-\mathbf{x}_j(t))
\delta (\mathbf{v}-\mathbf{v}_j(t)),
\end{eqnarray} 
%
which is inferred as $N^p$ particles with the positions $\mathbf{x}_j$, the velocity $\mathbf{v}_j$, and the particle weight $w_j$.
However, as indicted previously, these marker particles may be simply Monte Carlo samples of the particle distribution function, for example. %so, in this sense, there is no direct relation among the physical atomic particles in the plasma and this $N^p$ marker distribution function.

%\todo{Danial: Bob doesn't like the above equation due to presence of delta functions. Although this notation is not typical for statisticians, this type of presenting a distribution function is common in the particle filter literature. Also I believe having this equation in this paper helps to connect to physics community and avoid confusions (e.g. CPC reviewers) wrt the imposed constraints.}


==> paper_4_temp.tex <==
% Opening

In this section we present several numerical examples motivated by the
use of MPCR in \blue{full-$f$ gyrokinetic simulations}. In these
examples, the constrained optimization problem (\ref{eq:quadprog}) is
solved using the \blue{well-established} algorithm of Goldfarb \& Idnani \cite{goldfarb1983}
as implemented in the \textit{quadprog} library \cite{quadprog}. 
\blue{There are numerous other optimization algorithms that could
be used for this straight-forward quadratic programming problem.}
%In general, the quadratic (or convex) programming calculations required in MPCR can be performed
%using any optimization algorithm.


In the first set of test problems, we demonstrate the ability of MPCR
to preserve features of the distribution function when resampling an
arbitrary distribution and resampling particles from an XGC plasma
turbulence solution. Finally we show the benefits of periodic particle
resampling using MPCR on \blue{the well-known Landau damping problem
as well as} a neoclassical tokamak plasma simulation.  \blue{In a
neoclassical simulation, transport is represented by a diffusion
process that is forumated to account for the effects of the magnetic
geometry, which may produce complex particle orbits and drifts.}

\subsection{Global resampling examples}

%===============================================================
% Non-Maxwellian local features preservation (1D)
%
%\begin{figure}[h!]
%\centering
%	\includegraphics[trim = 0mm 0mm 0mm 0mm, clip, width=.48\textwidth]{figures/initial_f_maxwell_bar.png}
%	\\ \vspace{-0.1in}
% 	\caption{Initial particle distribution function with local features. In this case, total number of particles $N^p$ is 50000.
% 	         The solid red curve is a Gaussian.}	
%	\label{fig:1d_localfeature}
%\end{figure}
% 

\begin{figure}[tp]
\centering
	\includegraphics[trim = 140mm 0mm 140mm 0mm, clip,width=.48\textwidth]{figures/initial_f_maxwell_bar.png}
        ~
        \includegraphics[trim = 140mm 0mm 140mm 0mm, clip,width=.48\textwidth]{figures/downsampled_dsf200.png}
	\\ \hspace{0.0in} (a) \hspace{2.6in}
	  (b) \\
          \includegraphics[trim = 140mm 0mm 140mm 0mm, clip,width=.48\textwidth]{figures/random_dsf50.png}
	  ~
          \includegraphics[trim = 140mm 0mm 140mm 0mm, clip,width=.48 \textwidth]{figures/random_dsf200.png} \\ \hspace{0.0in}
	  (c) \hspace{2.6in} (d) \vspace{-0.1in}
          \caption{Synthetic
	  distribution $f$ \blue{as a function of general phase space
        variable $\alpha$}, as represented initially by $N^p=50000$
	  marker particles, and down-sampled by a factor 50 and 200,
	  using MPCR and global random down-sampling. The MPCR algorithm is
	  applied with 50 bins, which are the same as the bins used
	  in the histograms. Shown are:
          (a) initial distribution,
          (b) MPCR with $\mathrm{DSF}=200$ 
          %($\mathrm{DSF}=50$ is identical by construction)
          , and global random down-sampling with (c) $\mathrm{DSF}=50$ and
          (d) $\mathrm{DSF}=200$. In (a), the curve is a Gaussian.}	
	\label{fig:1d_localfeature_dsf}
\end{figure}
%
%In current XGC implementations, the particle down-sampling process for multi-fidelity simulations is performed by randomly choosing particles over the entire domain of $f$, without preserving any features, or moments, of the system.  Subsequently, one might anticipate that MPCR would provide a significant improvement in the accuracy of the kinetics representation.  Using this as motivation, 

For the first example, consider the one-dimensional probability
distribution represented by the histogram shown in
Figure \ref{fig:1d_localfeature_dsf}(a). It might, for example, be a
distorted marginal distribution of one of the velocity components. In
this case, Maxwell-Boltzmann statistics would yield a Gaussian
distribution, and the given distribution is clearly far from Gaussian.
\blue{
In this figure, the synthetic distribution function $f$ is presented
as a function of a general phase space variable $\alpha$,
which could, for example, be any velocity or position coordinate of the phase space.
}
This distribution is represented with $N^p=50000$ samples \blue{with non-uniform weights generated from a perturbed Gaussian,
%distribution on [% of ??}\todo{RDM: is this correct? it's to address item 5 of
%reviewer 1, what is the weight?}, 
and down-sampled to $M^p=1000$ and $M^p=250$: down-sampling factors (DSF)
of 50 and 200, respectively.}
%

Down-sampling was performed using MPCR in one-dimension, using
$M^b=50$ bins in which the sample density, and first and second
moments are preserved.  For comparison, global random down-sampling
was also used\blue{, in which $M^p$ new marker particles are selected randomly from the $N^p$ old 
particles. Such global down-sampling has been used in the past in
plasma PIC codes, for example, in the
XGC plasma simulation codes.}
The results are shown in
Figures \ref{fig:1d_localfeature_dsf} and \ref{fig:1d_error}. By
construction, the histogram formed on the 50 down-sampling bins is
identical to that of the original sample, but the randomly down-sampled
histograms show large variations from the original.  Indeed, the
sampling error obscures the structure of the distribution; so much so
that in the DSF=200 case, the underlying structure of the distribution
is not visible at all. By construction, the low-order moments of the
distribution are preserved in MPCR, as shown in
Figure \ref{fig:1d_error}, whereas relative errors in the moments with
random down-sampling range from 2\% to 10\%. %\todo{RDM: please plot second moment errors also}
%
\begin{figure}[tp]
\centering
	\includegraphics[trim = 140mm 0mm 140mm 0mm, clip, width=.48\textwidth]{figures/1d_error_f_g.png}
%	~
%	\includegraphics[trim = 140mm 0mm 140mm 0mm, clip, width=.48\textwidth]{figures/1d_error_g.png}
	\caption{Relative error in global 0th and 1st moments due to feature-based/random down-sampling for different down-sampling factors
	(error in random down-sampling is the mean of $10^4$
	realizations).}
	%\todo{RDM: please include second moments.	
	\label{fig:1d_error}
\end{figure}
%

MPCR up-sampling was also tested on the distribution function from
Figure \ref{fig:1d_localfeature_dsf}(a), with similar results. That is,
constrained moments are preserved to roundoff error, while detailed features
of the distribution are preserved on the scale of the binning (not
shown). A common alternative up-sampling approach is particle
reproduction \cite{douc2005}, in which each particle is duplicated $n_u$
times, where $n_u$ is the up-sampling factor. This will obviously
preserve all moments and all features of the sampled distribution
function. However, if the subsequent evolution of the particles in the
PIC code is deterministic, it will accomplish nothing, since the
particles will remain identical for all time and not provide an
improved sample of $f$. To avoid this, some algorithms perturb the
position and/or the velocity of the duplicated particles \cite{douc2005},
which without further adjustment results in the target moments not
being preserved. As the duplicated and perturbed particles evolve,
they will commonly diverge from one-another (assuming the particle
evolution is chaotic), and become independent samples of the
distribution after some time, with the divergence rate governing how
long this takes. Similarly, if particle evolution is stochastic, then
exactly duplicated particles will also diverge, and also become
independent samples of the distribution over time. In contrast, by
sampling from a binned approximation of $f$ and imposing a set of
integral constraints, MPCR up-sampling produces nearly independent
samples immediately.


%===============================================================
% 4D results

For a second example, the resampling algorithm is applied to the
particle distribution taken from a tokamak plasma simulation
performed with the gyrokinetic PIC code XGC1.
%
In a spatially three-dimensional gyrokinetic PIC code, each particle
is characterized by six attributes, its weight $w$, spatial
coordinates $\mathbf{x} = (r;z;\phi)$, and velocity coordinate
$\mathbf{v} = (v_\|; v_{\perp})$. In this example, the distribution
$f$ is projected on to a spatially two-dimensional configuration space
in $r$ and $z$, taking advantage of statistical homogeneity in
$\phi$. The motivation for this aspect of the test, is to enable the
projection of a solution from a spatially three-dimensional plasma
turbulence simulation to serve as an initial condition for a
two-dimensional neoclassical simulation.  The data set consists of
$N^p=10^6$ particles, initially weighted to effect importance
sampling, as discussed in Section~\ref{sec:method}. However, particles
have since been mixed through their evolution, so their weights no
longer accomplish the desired importance sampling.
%
\begin{figure}[tp]
\centering
	\includegraphics[trim = 120mm 0mm 140mm 0mm, clip, width=.48\textwidth]{figures/weight_new.png}
	~
	\includegraphics[trim = 120mm 0mm 140mm 0mm, clip, width=.48\textwidth]{figures/UP_weight_hist_new.png}
\\  \hspace{0.0in} (a) \hspace{2.5in} (b) \vspace{-0.1in}
	\caption{
	Histograms of particle weights from the original
	weights and the proposed resampling algorithm. 
	In this case $N^p=10^6$ and the number of bins
	in the  $\rho$, $\mu$, $r$ and $z$ directions is 50:
	(a) original particles and downsampled particles with down-sampling factor (DSF) = 20,
	(b) upsampled particles with up-sampling factor (USF) = 10.}	
	\label{fig:hits_w}	
\end{figure}
%

The first step of the particle resampling process is to divide the
four-dimensional phase space $\boldsymbol{\zeta}$ into bins and sort
the particles into those bins.  In the gyrocentered XGC1 code, the
particle velocity space is parameterized in terms of the normalized
parallel velocity $\rho=v_\|/B$ and magnetic moment
$\mu=v_\perp^2/2B$, where $B$ is the magnitude of the magnetic
field. For this case then, the four-dimensional down-sampled phase
space is $\boldsymbol{\zeta}=(r,z,\rho,\mu)$. The $\boldsymbol{\zeta}$
domain is divided into bins, with 50 bins in each of the four
phase-space directions.

\blue{To demonstrate the adjustment of weights as part of the resampling
process the importance weighting is eliminated by making $g \propto
f$, where $g$ is the marker particle distribution function
in \eqref{eq:targetM} to enforce uniform target weights in bins.
}
The target number of particles $M^p_i$ in each
bin is then simply proportional to the sum of the weights of the
original particles in the bin. Specifically,
%
\begin{equation}
M^p_i=M^p\left(\frac{\sum_{j=1}^{N_i^p} w^i_j}{\sum_{j=1}^{N^p} w_j}\right).
\end{equation} 
%

One complication that arises in sorting the particles into bins is
that in some cases the target number of down-sampled particles $M^p_i$
in a bin is too small to allow the constraints to be imposed. In this
case, neighboring bins in the velocity space directions $(\rho,\mu)$
are merged to form larger bins with more particles, until $M^p_i$
exceeds a specified minimum, which was set here to $M^p_i \geq 25$.

The distribution of particle weights is shown in
Figure~\ref{fig:hits_w} for the original particles, and for the result
of down-, and up-sampling using the MPCR algorithm. Note that the
original distribution is broad, while the resampled distributions are
strongly peaked. The target marker particle distribution for both
cases was to eliminate importance sampling and make the weights
uniform. The fact that the resampled weight distributions are not
delta-functions is a consequence of the weight adjustments used to
preserve moments. The down-sampled particle weights are much larger
than the original weights and the up-sampled weights are much smaller
because the mean of the weights must increase (decrease) by the
down-scaling (up-scaling) factor.  Also by construction, the features
of the distribution in both space and velocity are preserved after
resampling. % (Figure~\ref{fig:f_2d_hits}).


The accuracy of the moment preservation in the resampling approach is
tested by down-sampling while preserving different moments.  Three
cases were considered: preserving 1) the zeroth moment, 2) the zeroth
and first moments, and 3) the zeroth through second moments, as
described in Section~\ref{sec:method}. This was done for a range of
down-sampling factors, and resulting errors in the moments are shown in
Figures \ref{fig:error_dsf}, along
with errors for random down-sampling. The moment errors for the random
down-sampling are averaged over $10^4$ sampling realizations.
%
\begin{figure}[tp]
\begin{center}
%\hfill	
\includegraphics[trim = 120mm 0mm 140mm 0mm, clip, width=.34\textwidth]{figures/f.png}%
~
\includegraphics[trim = 150mm 0mm 140mm 0mm, clip, width=.31\textwidth]{figures/g_mu.png}
~
\includegraphics[trim = 150mm 0mm 140mm 0mm, clip, width=.31\textwidth]{figures/h_mu.png}
\end{center}
\caption{Relative error in global zeroth, first and second velocity
	space moments as a function of down-sampling factor, using
	random down-sampling and MPCR down-sampling constrained to
	preserve zeroth, up to first and up to second moments.  Errors
	in configuration space moments are similar. There were
	$N^p=10^6$ original particles extracted from XGC1, and there
	were 10 bins in the $\rho$, $\mu$, $r$ and $z$ directions, for
	a total of $10^4$ bins.}  \label{fig:error_dsf}
\end{figure}
%

There are several interesting features of these errors. First, as
expected, the relative errors in the moments that are preserved are
order $10^{-10}$ or less. Second, with the MPCR algorithm, even the
moments that are not constrained have significantly lower errors than
for random sampling, in some cases by three orders of magnitude. This
improvement over random sampling is presumably due to the binning,
which enforces a descrete representation of the global distribution that
defines the moments. \blue{Notice in particular that the error in the second
moment when constraining the first moment is only marginally better
than when just the zeroth moment is constrained.}
Finally, for both random down sampling and for
unconstrained moments in MPCR, the relative error increases with
down-sampling factor. The observed weak growth is as expected for
random sampling, which should introduce errors that scale with the
square root of the down-sampling factor. In contrast the relative
errors in the unconstrained moments in MPCR grow much more rapidly
with down-sampling factor.

%

%% UPSAMPLING error
The reduction of errors relative to random down-sampling due to
binning, as discussed above, suggests that in MPCR, moment errors should
reduce with increasing bin density. This is indeed the case, as
shown in Figure~\ref{fig:UPerror_bin}, where relative error in an
up-sampling case is plotted as a function of the number of bins in
each direction. The error in the first moment when only the zeroth
moment is constrained appears to be decreasing like the number
of bins in each direction squared. Recall that the up-sampling
algorithm involves sampling a uniform distribution on each bin. As
mentioned in Section~\ref{sec:method}, more sophisticated sampling in
each bin can be used, which could result in a more rapid reduction of
errors with number of bins. Finally note that as with down-sampling,
preserved moments have relative errors that are better than $10^{-10}$.


\begin{figure}[!t]
\begin{center}
	\includegraphics[trim = 0mm 0mm 0mm 0mm, clip, width=.32\textwidth]{figures/UPg_rho.png}%
	\includegraphics[trim = 0mm 0mm 0mm 0mm, clip, width=.32\textwidth]{figures/UPg_mu.png}
	\includegraphics[trim = 0mm 0mm 0mm 0mm, clip, width=.31\textwidth]{figures/UPg_zero_momemnts.png}	
\end{center}
\caption{Relative
	error in global first moments in $\rho$ and $\mu$ as a
	function of the number of bins in each direction, $\rho$,
	$\mu$, $r$ and $z$.  MPCR up-sampling was used,
	constrained to preserve zeroth, up to first and up to second
	moments.  There were $N^p=10^6$ original particles extracted
	from XGC1, and the up-scaling factor was 10.  $E(\mu)\approx N^{-2.1}$ and $E(\rho)
	\approx N^{-2.7}$, where $N$ is the number of bins and $E(\cdot)$ is the error in the corresponding moment.	%\todo{RDM: please
	%include a third plot with the relative error in the first moment of
	%$\rho$ and $\mu$ from the 0-moment case, ploted on a log-scale
	%that shows the variation of the error as a function of
	%bin \#. We should be able to estimate the order of convergence.}
	% Danial: The 3rd plot is added in log-log. The equations for the fites are
	% \int \rho f => y = -2.7x + 6.6
	% \int \mu f  => y = -2.1x + 4.4	
	% where x = log (number of bins) and y = log (relative error)
	}
	\label{fig:UPerror_bin}	
\end{figure}
%




%===========================================================================================================
% 				Landau damping simulations PROBLEM 
%===========================================================================================================
\subsection{\blue{Periodic particle resampling in Landau damping}}
\blue{
In this section, the MPCR algorithm is applied to as simulation of the
linear regime of a Landau
damping \cite{Landau} test case. Landau damping is a phenomenon in
which the oscillations of the number density of particles in a
collisionless plasma are exponentially damped. This is a
well-known plasma physics phenomenon, confirmed in both
experiments \cite{Derfler} and
simulations \cite{myers2017,chacon2016}.  For this test case, a
full-$f$ PIC code in one spatail and velocity dimension as implemented
by \cite{pic_landaudamp} is applied to the Landau damping problem. In all
simulations, the initial distribution function of particles is taken
to be uniform in space ($x \in [0,2\pi/k]$) and Maxwellian in
velocity, while the particle weights are selected to enforce the
initial condition
\begin{equation}
  f(\mathbf{x},\mathbf{v}, t=0) = \frac{1}{2\pi}\left(1+\varepsilon \cos(kx)\right)\exp\left(-\frac{v^2}{2v_{th}^2}\right),
\end{equation}
where $k=0.5$ and the perturbation $\varepsilon=0.05$ is chosen to
ensure the perturbation is in the linear regime.
The simulations are performed using a grid of $50\times50$ cells and a
time step of 0.1.  The in the units of the problem, the thermal
velocity $v_{th}$, phase velocity $v_p$, and plasma frequency
$\omega_p$ are all one.\todo{RDM:How do $v_p$ and $\omega_p$ enter the
definition of the problem, why can you just define them to be one?
$\omega_p$ appears to arrise from the solution.}
The numerical conservation of the the time evolution of the electric field $\mathbf{E}$ is considered here as a measure of the PIC simulation accuracy. An (approximate) analytical solution of the electric field, valid in the small $\varepsilon$ regime can be derived through a linear approximation of the Vlasov-Poisson equation \cite{sonnendrucker2010}.  This yields an approximation to the total electrostatic energy at time $t$ of
\begin{equation} 
E(t) \propto E_0 ~ Re(e^{i \omega (t - \alpha)})^2, \quad E_0 = \frac{\pi \varepsilon}{2 k^3}
\end{equation}
where $E_0$ is the inital electrostatic energy, $\alpha$ is selected so that $E(0)=E_0$, and the complex-valued $\omega$ is the root of the dispersion relation,
\begin{equation}
1+\left( \frac{\omega_p}{v_{th} k} \right)^2 \left(1+ \frac{\omega}{\sqrt{2} v_{th}k} Z(\frac{\omega}{\sqrt{2} v_{th}k}) \right)  =0, \quad Z(x) = \sqrt{\pi} e^{-x^2} (i-\text{erfi}(x)
\end{equation}
For $k=.5$, $\omega \approx 1.415661888604536 - 0.153359466909605i$.
Therefore, one can compare the numerical solution of the $L^{2}$-norm of the electric field (electric field energy) with the the analytical approximation.}

The PIC simulations of  Landau  damping indicates that the computed electric field energy match the analytical approximation over longer time frames for simulations with a higher number of marker particles \cite{chacon2016}. This is because in the PIC simulation with low number of particles, the initial marker distribution rapidly becomes inhomogeneous and particle weights no longer accomplish the importance sampling. Performing periodic resampling using MPCR can reduce this unfavorable effect through conserving the desired marker particle distribution and importance sampling weights. Figure \ref{fig:Ldamp} compares the time evolution of the electric field energy obtained from the analytical approximations with the ones computed from the PIC simulations using 1 million and 50 million marker particles as well as a simulation with 1 million particles with periodic resampling. The particle resampling  is conducted every 20 timesteps by constraining the zeroth and first moments in velocity and position. These numerical experiments indicate that increasing the number of simulation particles results in the computed electric field energy match to the analytical solution over longer time frames.  However, after $t \approx 15$ the rate of oscillation damping decreases in the 1 million particle simulation and a drift in the oscillation frequency appears with respect to the analytical approximation. However, periodic particle resampling on the 1 million particle simulation increases accuracy %conserves the importance sampling by readjusting the particle weights
and leads to a computed electrostatic energy closer to both the analytical solution as well as the 50 million (50x) particle simulation. 
As a measure of the discrepancy between the computed electrostatic energy, Figure \ref{fig:Ldamp} shows the $L^2$ error norms with respect to the 50 million particle simulation.

\begin{figure}[tp]
\centering
	\includegraphics[trim = 0mm 0mm 0mm 0mm, clip, width=.49\textwidth]{figures/Landaudamp_E.png}%		
	~
	\includegraphics[trim = 0mm 0mm 0mm 0mm, clip, width=.49\textwidth]{figures/Landaudamp_L2error.png}%		
	\caption{\blue{Time evolution of the electric field energy in Landau  damping simulations with 1 and 50 million particles without resampling, and 1 million particle with periodic resampling every 2 second. Time evolution of the $L^2$ error of the 1 million particle simulation with and without resampling. }} % with respect to  50 million  particle simulation.}}
	\label{fig:Ldamp}
\end{figure}


%==================================================================================================================
% 				XGCa NEO-CLASSICAL TEST PROBLEM 
%==================================================================================================================
\subsection{Periodic particle resampling of a neo-classical PIC simulation}


%===== Robert Hager's paragraph ===========================================================================
\blue{
XGCa \cite{hager2016_1,sku_2016,sku_2009} is a global gyrokinetic
particle-in-cell (PIC) code with an axisymmetric electrostatic
potential solver specialized for the simulation of neoclassical
transport physics in the edge plasma of toroidal magnetic confinement
devices.  These simulations are capable of evolving the full
five-dimensional gyrocenter distribution function from the magnetic
axis to the inner wall of the device using either conventional
full-$f$ (constant particle weight) \cite{sku_2009} or
total-$f$ (variable particle weights) \cite{sku_2016} methods.  
% -------------- Removed to address the JCP reviewer's comment ----------------------------
%A logical sheath boundary condition \cite{parker1993suit} is used to
%prevent net currents to the material wall.  Plasma lost to the
%material wall is replenished self-consistently by a neutral particle
%recycling model according to the local loss rates.  Collisional
%physics are represented either by a fully nonlinear, Eulerian
%Fokker-Planck-Landau collision operator \cite{yoon_2014,hager2016_2}
%(total-$f$) or a linearized Monte Carlo collision
%operator \cite{wwang_1999} (full-$f$).
}

As a proof-of-principle test, the impact of the MPCR algorithm on
several important characteristics of the simulated plasma are
investigated here; particularly the radial electric field that is needed to
maintain quasi-neutrality, the maintenance of a divergence-free equilibrium
plasma flow, and the conservation of toroidal angular momentum.  For
simplicity, we use the full-$f$ representation of a single ion species (deuterium) with
the adiabatic electron model.
%

\blue{
The magnetic equilibrium field is that of a generic, up-down
symmetric, low-aspect ratio tokamak with a circular boundary surface
and Shafranov shift.  
% -------------- Removed to address the JCP reviewer's comment ----------------------------
%Since no material wall is included in the
%simulation, particles that leave the simulation region at the outer
%boundary are re-inserted into the simulation on the same flux-surface
%but at the poloidal angle, at which they would have re-entered the
%simulation domain had they been allowed to continue their orbit.
Marker particles are initiated with a uniform distribution in
configuration and velocity space and perpendicular and parallel
velocities of up to approximately $3.5 v_{th}$, where $v_{th}$ is the
thermal velocity.  The marker particle weights $w$ are set to produce
a locally Maxwellian distribution with density $n_i(\psi)$ and
temperature $T_i(\psi)$ that depend only on the flux-label
(generalized minor radial coordinate) $\psi$; that is, each particle's
initial weight is a function of its initial flux-label and velocity.
The electrostatic potential is initially zero.
}

\begin{figure}[tp]
\centering
	\includegraphics[trim = 120mm 0mm 120mm 0mm, clip, width=.36\textwidth]{figures/xgca_figs/MarkerDensity_50m_ts0.png}%			
	\includegraphics[trim = 150mm 0mm 120mm 0mm, clip, width=.33\textwidth]{figures/xgca_figs/MarkerDensity_50m_ts6000.png}%
\includegraphics[trim = 150mm 0mm 100mm 0mm, clip, width=.345\textwidth]{figures/xgca_figs/MarkerDensity_Res_ts6000.png}
	\caption{Spatial distribution of particle density for the
	simulation with 50 million particles: initial particle
	distribution (left), at $t=12\tau_t$ without resampling
	(middle), and at $t=12\tau_t$ with resampling (right).}	
	\label{fig:DensityDist}
\end{figure}

%
A local Maxwellian is, however, not the neoclassical equilibrium
distribution in the presence of a pressure gradient, due to the
magnetic inhomogeneity drift, which causes charged particles in
tokamaks to move on so-called banana-orbits with finite width.
Starting with a local Maxwellian distribution and
vanishing radial electric field, the orbital motion of the ions, together
with the background pressure gradient leads to the development of an
up-down anti-symmetric pressure variation and a net toroidal
flow. If this were the equilibrium flow it would
violate the divergence-free condition
and toroidal angular momentum conservation.  To make the
equilibrium flow divergence free and cancel the net toroidal flow from
the magnetic inhomogeneity drift, the plasma reacts by generating a
radial electric field (guiding center polarization) with its
corresponding $\mathbf{E}\times\mathbf{B}$ flow.
%


The challenge in calculating the radial electric field with a
full-f PIC code, arises because the orbital motion of the markers
leads to mixing of particles with disparate weights.  This is a
considerable source of sampling error, especially in regions with
small pressure gradient and low amplitude of the electrostatic
potential.  The purpose of periodic particle-resampling is to reduce
the sampling error by locally homogenizing the particle weights \blue{and by
improving the distribution of marker particles in phase space.}  We
demonstrate this capability by comparing the time evolution of the
radial electric field and the radial electric field profile in
quasi-steady state between simulations with a total of 5 million, 50
million, and 500 million marker particles without particle
re-sampling, and a simulation with 50 million particles with periodic
resampling.
%===== Robert Hager's paragraph ===========================================================================
\begin{figure}[t]
\centering	
	\includegraphics[trim = 120mm 0mm 120mm 0mm, clip, width=.33\textwidth]{figures/xgca_figs/Er3D_5m_cnt.png}%
	\includegraphics[trim = 120mm 0mm 120mm 0mm, clip, width=.33\textwidth]{figures/xgca_figs/Er3D_50m_cnt.png}%
	\includegraphics[trim = 140mm 0mm 140mm 0mm, clip, width=.33\textwidth]{figures/xgca_figs/Er3D_50m_srf.png}\\			
	\includegraphics[trim = 120mm 0mm 120mm 0mm, clip, width=.33\textwidth]{figures/xgca_figs/Er3D_500m_cnt.png}%
	\includegraphics[trim = 120mm 0mm 120mm 0mm, clip, width=.33\textwidth]{figures/xgca_figs/Er3D_50mRes_cnt.png}%	
	\includegraphics[trim = 140mm 0mm 140mm 0mm, clip, width=.33\textwidth]{figures/xgca_figs/Er3D_50mRes_srf.png}	
\caption{Spatio-temporal evolution of $E_r$ in simulations with 5, 50
	and 500 million particles without resampling and 50 million
	particles with resampling.}	
	\label{fig:Er3d_5_50_500M}
\end{figure}

In all cases, the PIC simulations are run for 12 toroidal transit
times ($\tau_t$),
which is sufficient for the equilibrium plasma flow to
develop. 
% 6000 time steps of 0.002 of the toroidal transit time.
The spatial marker particle density is intended to be approximately
uniform through the core and edge plasma to yield a good
representation of the low-density edge region. However, as the plasma
evolves the particles mix and the initial marker distribution becomes
inhomogeneous, spoiling the intended importance sampling. This is
apparent in Figure~\ref{fig:DensityDist}, in which the initial and
final marker particle densities for the 50 million particle case are
plotted (no resampling). A similar mixing occurs in velocity space,
which would spoil any importance sampling used, for example, to represent high
energy ions. The result of
this poor sampling of the particle distribution is that large Monte Carlo
sampling error is introduced into the simulation. As an example,
consider the spatio-temporal evolution of the radial electric field
(Figure \ref{fig:Er3d_5_50_500M}) for the 5, 50 and 500 million
particle cases (no resampling).  In all three cases, the error is
largest in the edge region, $0.8< \psi <1$, \blue{where it manifests as
spurious oscilations,} because the marker
particle densities are low in this region. Further, \blue{the magnitude of
these oscilations} is reduced with increasing number of 
particles. Particularly, the oscilation magnitude decreased by about a
factor of $\sqrt{10}$ going from 50M and 500M particles, which is the
expected asymptotic convergence rate for errors dominated by sampling
error.


% resampling stages=============================================================================

To reduce the sampling error, the MPCR algorithm was applied
periodically in the 50 million particle simulation, in this case every
3 toroidal transit times ($3\tau_t$). There are 1500 times steps
between resamples, and the computational cost of resampling is
negligible compared to the time advance for this number of steps.  As
described in Section~\ref{sec:XGCimp}, the 2-dimensional unstructured mesh in
XGC is used for the configurational space bins consists of 6368 elements, and in velocity space 100
uniform bins were used in both the $v_\parallel$ and $v_\perp$
directions. At each resampling, the total number of marker particles
remained the same ($M^p=N^p$), and the target number of particles in
each bin is consistent with the initial marker particle distribution
(at $t=0$).

%
%
\begin{figure}[tp]
\centering
	\includegraphics[trim = 110mm 0mm 130mm 0mm, clip, width=.45\textwidth]{figures/xgca_figs/avgEr_phi2D.png}	
	~	
	\includegraphics[trim = 110mm 0mm 130mm 0mm, clip, width=.45\textwidth]{figures/xgca_figs/Er_t_psi8.png}
	\\
	\includegraphics[trim = 110mm 0mm 130mm 0mm, clip, width=.45\textwidth]{figures/xgca_figs/Er_t_psi2.png}
	~
	\includegraphics[trim = 110mm 0mm 130mm 0mm, clip, width=.45\textwidth]{figures/xgca_figs/Er_t_psi5.png}
	\\
	\hspace{0.2in}
	\includegraphics[trim = 0mm 0mm 0mm 0mm, clip, width=.45\textwidth]{figures/L2error_Er_t_psi2.png}
	~
	\includegraphics[trim = 0mm 0mm 0mm 0mm, clip, width=.45\textwidth]{figures/L2error_Er_t_psi5.png}				
	\caption{
	$E_r$ profile at 6000 time steps. 
	Time evolution of $E_r$ at $\psi = 0.5$, $\psi = 0.2$, $\psi = 0.8$.
	\blue{Time evolution of the pointwise error in simulations with 50 million particles with and without periodic resampling
	at $\psi = 0.2$ and $\psi = 0.5$, relative to the 500 million
	particle simulation.}} \label{fig:Er1d}	
\end{figure}
%
As a result of the periodic resampling, the marker particle
distribution in configuration space at the end of the simulation is
much more uniform than without the resampling
(Figure~\ref{fig:DensityDist}). This leads to much smaller oscilations in the
radial electric field $E_r$ (see
Figure~\ref{fig:Er3d_5_50_500M}). The resampled and non-resampled cases
are identical until the first resampling at $t=3\tau_t$. After the
resampling the oscilations in $E_r$ are immediately reduced.  Indeed, it is
reduced to levels comparable to the 500M particle non-resampled case,
as can be seen in Figure~\ref{fig:Er1d} where the time evolution of
$E_r$ at several points in $\psi$ is plotted for the both 50 million
particles cases (resampled and not) and the 500 million particle
case. Also shown is the $E_r$ profile as a function of $\psi$ averaged
over the period $4\tau_t<t<12\tau_t$, and the profile from the 50
million particle resampled case is a much more accurate approximation
of the 500 million particle profile than the non-resampled case.
\blue{As a measure of the discrepancy, Figure~\ref{fig:Er1d} shows the
$L^2$ error in $E_r$ relative to the 500 million marker particle simulation.}

After each resampling the errors grow slowly as can be seen
between the resamplings at $t=6\tau_t$ and $9\tau_t$. However, in the
initial period, the \blue{errors and oscilation amplitude} grow rapidly so that by $t\approx 3\tau_t$,
the they reach the magnitude maintained throughout the
non-resampled simulation. This is presumably due to the relatively
rapid evolution of the system toward the equilibrium plasma flow,
which could rapidly mix the particles in both configuration and
velocity space. Apparently once the flow is near equilibrium, the
mixing rates are more modest resulting in slower growth of the
sampling errors. This suggests that rather than resampling at a fixed
frequency, it would be useful to resample locally and adaptively based
on local estimates of the sampling errors. This would be particularly
useful in simulating transient phenomena, and could adaptively
determine the required number of particles to attain a specified
sampling error tolerance.


In PIC simulations, the primary computational cost is the evolution of
particles, and the relative cost of periodic particle resampling in a
plasma PIC simulation will be small.  %To see this, consider that the
%cost of binning the particles is similar to the cost of the charge
%deposition step that occurs every timestep to compute electromagnetic
%fields.  
\blue{
The main expense in resampling is the solution and setup of the quadratic program. The dominant cost 
there is the QR factorization of the constraint matrix.  This cost scales quadratically with the number of constraints. For the XGCa test case given above, this results in a computational complexity 
roughly 20 times that of a typical XGCa timestep(using an explicit RK4 time integrator).   Given that the resampling occurs 3 times over 6000 total timesteps, the resampling overhead is roughly 1\% of the total simulation cost.   In addition, given a spatial decomposition of particles across MPI processes, a typical
PIC timestep involves an allgather for the charge density, a broadcast of the resulting electric field, and 
the shifting of particles(via sends and receives) from one MPI process to another.  In this scenario, the resampling algorithm is completely local and has no communication overhead.  Capturing these communication costs for accurate timing information requires a full integration of the resampling algorithm into the XGCa framework, which is currently in the software development stage.}

%factorization, for each bin, of a matrix with dimension the number
%of resampled particles in the bin by the number of equality
%constraints (of order 25 in the XGCa example, depending on the grid
%geometry).\todo{RDM: Is this why the number quoted is only
%approximate?, if not, please fix} This expense is certainly less than,
%for example, the cost of the global solution for the electrostatic
%potential $\phi$ via a direct (or iterative) solver, which occurs
%every time step.\todo{Is this really true? it's not obvious to me. Can
%we time the computations (not the I/O) in Danial's resampling code,
%and scale it to compare to the cost of a time step in the XGCa case?
%Thus, applying the resampling algorithm costs
%ess than a single time step of the PIC simulation, and
%since it needs to be done infrequently, this cost is negligible. 
The
results presented here indicate that application of MPCR will allow
significantly fewer particles to be used to attain the same accuracy,
thereby reducing the cost of PIC simulations, which scale
approximately with the number of particles.
























